Fusion-GCN: Multimodal Action Recognition using Graph Convolutional Networks

In this paper, we present Fusion-GCN, an approach for multimodal action recognition using Graph Convolutional Networks (GCNs). Action recognition methods based around GCNs recently yielded state-of-the-art performance for skeleton-based action recognition. With Fusion-GCN, we propose to integrate various sensor data modalities into a graph that is trained using a GCN model for multi-modal action recognition. Additional sensor measurements are incorporated into the graph representation, either on a channel dimension (introducing additional node attributes) or spatial dimension (introducing new nodes). Fusion-GCN was evaluated on two public available datasets, the UTD-MHAD- and MMACT datasets, and demonstrates flexible fusion of RGB sequences, inertial measurements and skeleton sequences. Our approach gets comparable results on the UTD-MHAD dataset and improves the baseline on the large-scale MMACT dataset by a significant margin of up to 12.37% (F1-Measure) with the fusion of skeleton estimates and accelerometer measurements.

==> author-citation.tex <==
\makeatletter
\newcommand\keyauthormap[2]{%
  \@namedef{keyauthormap-#1}{#2}%
}
\newcommand\acite[1]{%
  \@nameuse{keyauthormap-#1} \cite{#1}%
}
\keyauthormap{DBLP:conf/icvgip/ForoughiRP08}{Foroughi, Rezvanian and Paziraee}
\keyauthormap{DBLP:journals/air/RamezaniY16}{Ramezani and Yaghmaee}
\keyauthormap{DBLP:journals/corr/abs-1708-03805}{Bian et al.}
\keyauthormap{DBLP:conf/aaai/YanXL18}{Yan, Xiong and Lin}
\keyauthormap{DBLP:conf/cvpr/ShiZCL19a}{Shi et al.}
\keyauthormap{luciani:hal-00980003}{Luciani}
\keyauthormap{DBLP:conf/bmvc/ThakkarN18}{Thakkar and Narayanan}
\keyauthormap{DBLP:conf/cvpr/LiCCZW019}{Li et al.}
\keyauthormap{DBLP:books/sp/17/Asadi-AghbolaghiCBEPBGKE17}{Asadi-Aghbolaghi et al.}
\keyauthormap{Novack2017}{Novack and Goldin-Meadow}
\keyauthormap{Cartmill2012}{Cartmill, Beilock and Goldin-Meadow}
\keyauthormap{DBLP:journals/csur/AggarwalR11}{Aggarwal and Ryoo}
\keyauthormap{DBLP:conf/nips/LanWYM10}{Lan et al.}
\keyauthormap{Smyth2013}{Smyth and Wing}
\keyauthormap{DBLP:conf/icip/ChenJK15}{Chen, Jafari and Kehtarnavaz}
\keyauthormap{DBLP:journals/corr/ShahroudyLNW16}{Shahroudy et al.}
\keyauthormap{DBLP:journals/corr/abs-1806-11230}{Kong and Fu}
\keyauthormap{DBLP:conf/icmcs/NiuLHW04}{Niu et al.}
\keyauthormap{DBLP:journals/tip/HuXFZM07}{Hu et al.}
\keyauthormap{DBLP:conf/cvpr/NiYK09}{Ni, Yan and Kassim}
\keyauthormap{DBLP:journals/air/TripathiJA18}{Tripathi, Jalal and Agrawal}
\keyauthormap{DBLP:journals/access/GaoXXHLAJF18}{Gao et al.}
\keyauthormap{Noury2007}{Noury et al.}
\keyauthormap{DBLP:conf/iccvw/SolbachT17}{Solbach and Tsotsos}
\keyauthormap{DBLP:conf/cvpr/DuongBPV05}{Duong et al.}
\keyauthormap{Huynh2009}{Huynh et al.}
\keyauthormap{DBLP:conf/eccv/CiptadiGR14}{Ciptadi, Goodwin and Rehg}
\keyauthormap{DBLP:conf/hri/RyooFXAM15}{Ryoo et al.}
\keyauthormap{Soomro2014}{Soomro and Zamir}
\keyauthormap{DBLP:journals/cviu/LuoWH03}{Luo, Wu and Hwang}
\keyauthormap{DBLP:journals/cviu/BidhendiFSM17}{Bidhendi et al.}
\keyauthormap{DBLP:journals/corr/abs-1904-10354}{Kotyan et al.}
\keyauthormap{Zheng2018}{Zheng, Bao and Xu}
\keyauthormap{DBLP:journals/cviu/Gavrila99}{Gavrila}
\keyauthormap{DBLP:journals/corr/abs-1812-08008}{Cao et al.}
\keyauthormap{DBLP:conf/icml/NgiamKKNLN11}{Ngiam et al.}
\keyauthormap{DBLP:conf/aaai/PengHCZ20}{Peng et al.}
\keyauthormap{DBLP:conf/cvpr/LiuZC0O20}{Liu et al.}
\keyauthormap{DBLP:conf/iclr/KipfW17}{Kipf and Welling}
\keyauthormap{DBLP:conf/iccv/KongWDKTM19}{Kong et al.}
\keyauthormap{LeCun1998}{LeCun et al.}
\keyauthormap{Goodfellow-et-al-2016}{Goodfellow, Bengio and Courville}
\keyauthormap{Gori2005}{Gori, Monfardini and Scarselli}
\keyauthormap{DBLP:journals/tnn/ScarselliGTHM09}{Scarselli et al.}
\keyauthormap{Khamsi2011}{Khamsi and Kirk}
\keyauthormap{DBLP:journals/corr/LiTBZ15}{Li et al.}
\keyauthormap{DBLP:journals/corr/abs-1812-08434}{Zhou et al.}
\keyauthormap{Bruna2013}{Bruna et al.}
\keyauthormap{DBLP:conf/icml/NiepertAK16}{Niepert, Ahmed and Kutzkov}
\keyauthormap{DBLP:books/daglib/0080048}{Jain, Kasturi and Schunck}
\keyauthormap{DBLP:journals/corr/abs-math-0608522}{Hein, Audibert and von Luxburg}
\keyauthormap{DBLP:journals/spm/ShumanNFOV13}{Shuman et al.}
\keyauthormap{DBLP:journals/corr/HenaffBL15}{Henaff, Bruna and LeCun}
\keyauthormap{DBLP:conf/nips/DefferrardBV16}{Defferrard, Bresson and Vandergheynst}
\keyauthormap{DBLP:journals/corr/abs-0912-3848}{Hammond, Vandergheynst and Gribonval}
\keyauthormap{Chung1997}{Chung and Graham}
\keyauthormap{Mason2002}{Mason and Handscomb}
\keyauthormap{DBLP:journals/corr/abs-1912-06971}{Shi et al.}
\keyauthormap{DBLP:journals/vc/QinMLL20}{Qin et al.}
\keyauthormap{DBLP:conf/iccv/ZhaoWSJ19}{Zhao et al.}
\keyauthormap{DBLP:journals/neco/HochreiterS97}{Hochreiter and Schmidhuber}
\keyauthormap{Chung2014}{Chung et al.}
\keyauthormap{DBLP:journals/access/AhmadMLT20}{Ahmad et al.}
\keyauthormap{DBLP:journals/corr/abs-2003-07564}{Yang et al.}
\keyauthormap{DBLP:conf/iclr/ZophL17}{Zoph and Le}
\keyauthormap{DBLP:journals/corr/SimonyanZ14a}{Simonyan and Zisserman}
\keyauthormap{DBLP:conf/cvpr/Cheng0HC0L20}{Cheng et al.}
\keyauthormap{DBLP:journals/corr/abs-2003-03007}{Yang et al.}
\keyauthormap{DBLP:conf/mm/JiangY15}{Jiang and Yin}
\keyauthormap{DBLP:journals/corr/abs-2008-09747}{Ahmad and Khan}
\keyauthormap{DBLP:conf/nips/KrizhevskySH12}{Krizhevsky, Sutskever and Hinton}
\keyauthormap{DBLP:journals/corr/abs-2003-06156}{Memmesheimer, Theisen and Paulus}
\keyauthormap{DBLP:journals/corr/abs-2008-09748}{Ahmad and Khan}
\keyauthormap{DBLP:journals/corr/CheronLS15}{Ch{\'{e}}ron, Laptev and Schmid}
\keyauthormap{DBLP:journals/tcyb/CaoZZL18}{Cao et al.}
\keyauthormap{DBLP:conf/ijcai/CaoZZL16}{Cao et al.}
\keyauthormap{DBLP:conf/icmcs/SongLXZ018}{Song et al.}
\keyauthormap{DBLP:conf/iros/LiuQWZYL19}{Liu et al.}
\keyauthormap{DBLP:journals/corr/abs-1806-01810}{Wang and Gupta}
\keyauthormap{DBLP:journals/corr/abs-1806-07243}{Norcliffe-Brown, Vafeias and Parisot}
\keyauthormap{DBLP:journals/corr/PengWWQ14}{Peng et al.}
\keyauthormap{DBLP:journals/corr/abs-2008-01148}{Islam and Iqbal}
\keyauthormap{DBLP:journals/pr/LiXPCZS20}{Li et al.}
\keyauthormap{DBLP:journals/prl/FrancoMM20}{Franco, Magnani and Maio}
\keyauthormap{DBLP:journals/corr/VaswaniSPUJGKP17}{Vaswani et al.}
\keyauthormap{DBLP:journals/corr/abs-1711-11248}{Tran et al.}
\keyauthormap{DBLP:journals/corr/HeZRS15}{He et al.}
\keyauthormap{DBLP:journals/corr/abs-1807-05118}{Liaw et al.}
\keyauthormap{DBLP:journals/corr/KingmaB14}{Kingma and Ba}
\keyauthormap{Smith2019}{Smith and Topin}
\keyauthormap{DBLP:conf/iclr/LoshchilovH17}{Loshchilov and Hutter}
\keyauthormap{2019ISenJ..19.1862L}{{Liu}, {Kong} and {Jiang}}
\keyauthormap{DBLP:conf/cvpr/LiuY18}{Liu and Yuan}
\keyauthormap{DBLP:journals/corr/SzegedyLJSRAEVR14}{Szegedy et al.}
\keyauthormap{DBLP:journals/corr/abs-2012-11866}{Sun et al.}
\makeatother

